Disentangling Intrinsic Importance from Emergent Structure in Multi-Expert Orchestration

Multi-expert systems, where multiple Large Language Models (LLMs) collaborate to solve complex tasks, are increasingly adopted for high-performance reasoning and generation. However, the orchestration policies governing expert interaction and sequencing remain largely opaque. We introduce INFORM, an interpretability analysis that treats orchestration as an explicit, analyzable computation, enabling the decoupling of expert interaction structure, execution order, and functional attribution. We use INFORM to evaluate an orchestrator on GSM8K, HumanEval, and MMLU using a homogeneous consortium of ten instruction-tuned experts drawn from LLaMA-3.1 8B, Qwen3 8B, and DeepSeek-R1 8B, with controlled decoding-temperature variation, and a secondary heterogeneous consortium spanning 1B-7B parameter models. Across tasks, routing dominance is a poor proxy for functional necessity. We reveal a divergence between relational importance, captured by routing mass and interaction topology, and intrinsic importance, measured via gradient sensitivity: frequently selected experts often act as interaction hubs with limited influence, while sparsely routed experts can be structurally critical. Orchestration behaviors emerge asynchronously, with expert centralization preceding stable routing confidence and expert ordering remaining non-deterministic. Targeted ablations show that masking intrinsically important experts induces disproportionate collapse in interaction structure compared to masking frequent peers, confirming that INFORM exposes functional and structural dependencies beyond accuracy metrics alone. Our code is available at https://github.com/parmanu-lcs2/inform.

==> intro.tex <==

\section{Introduction}
Modern multimodal systems spend the same computation on a trivial lookup as on a
question requiring several rounds of perception and inference. This uniformity is
convenient but wasteful: most of the cost of a fixed high budget is consumed by the
minority of queries that were already easy. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting \cite{ghosh2026disentangling}, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. \citet{tang2024evoagent} was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word.

A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. Aperture instantiates this idea with three components: a typed record of evidence
gathered so far, a calibrated estimator of whether that evidence is \emph{sufficient}
to answer, and a policy that decides which action to take next or whether to stop.
The design is deliberately model-agnostic -- each specialist  is a frozen black box behind a uniform interface, so the control
layer can be studied and improved independently of any single backbone~\cite{ghosh2026disentangling}. Our code is available at \url{https://github.com/parmanu-lcs2}.

\begin{table}[t]
  \centering
  \caption{Accuracy and mean inference cost across four benchmarks. Cost is normalized to the fixed-budget baseline. Accuracy and mean inference cost across four benchmarks.}
  \label{tab:results}
  \small
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    \textbf{System} & \textbf{Params} & \textbf{Docs} & \textbf{Charts} & \textbf{Scenes} & \textbf{Cost}\\
    \midrule
    Fixed budget (large)   & 34\,B & 78.1 & 71.4 & 69.8 & 1.00\\
    Fixed budget (small)   & 8\,B  & 70.6 & 63.2 & 61.1 & 0.42\\
    Static routing         & 8\,B  & 74.9 & 67.8 & 65.4 & 0.58\\
    \textbf{Aperture (ours)} & 8\,B & \textbf{77.8} & \textbf{71.0} & \textbf{69.2} & \textbf{0.59}\\
    \bottomrule
  \end{tabular}
\end{table}
